Tractable Regularization of Probabilistic Circuits

Probabilistic Circuits (PCs) are a promising avenue for probabilistic modeling. They combine advantages of probabilistic graphical models (PGMs) with those of neural networks (NNs). Crucially, however, they are tractable probabilistic models, supporting efficient and exact computation of many probabilistic inference queries, such as marginals and MAP. Further, since PCs are structured computation graphs, they can take advantage of deep-learning-style parameter updates, which greatly improves their scalability. However, this innovation also makes PCs prone to overfitting, which has been observed in many standard benchmarks. Despite the existence of abundant regularization techniques for both PGMs and NNs, they are not effective enough when applied to PCs. Instead, we re-think regularization for PCs and propose two intuitive techniques, data softening and entropy regularization, that both take advantage of PCs' tractability and still have an efficient implementation as a computation graph. Specifically, data softening provides a principled way to add uncertainty in datasets in closed form, which implicitly regularizes PC parameters. To learn parameters from a softened dataset, PCs only need linear time by virtue of their tractability. In entropy regularization, the exact entropy of the distribution encoded by a PC can be regularized directly, which is again infeasible for most other density estimation models. We show that both methods consistently improve the generalization performance of a wide variety of PCs. Moreover, when paired with a simple PC structure, we achieved state-of-the-art results on 10 out of 20 standard discrete density estimation benchmarks.

==> tikz/tikzlibrarypc.code.tex <==
% Copyright 2016 by Nicola Di Mauro and Antonio Vergari
%
% This file may be distributed and/or modified
%
% under the GNU General Public License.
%
% See the files LICENSE for more details.

\usetikzlibrary{chains}
%\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage{pgfplots}
\usepackage{xparse}
%\usepackage{listofitems}

%\newif\iflabelleft

\newdimen\mywidth
\newdimen\myheight

\newcommand*{\IfStringInList}[2]{%
  \in@{,#1,}{,#2,}%
  \ifin@
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}

% sum node style
\tikzstyle{sum} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.west) -- (path picture bounding box.east);}, node distance=1]

% product node style
\tikzstyle{prod} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south east) -- (path picture bounding box.north west); \draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south west) -- (path picture bounding box.north east);}, node distance=1]

% \sumnode [tikz-options] {sum node name} 
\newcommand{\sumnode}[2][]{
  \node[sum, #1] (#2) {};
}

% \prodnode [tikz-options] {product node name} 
\newcommand{\prodnode}[2][]{
  \node[prod, #1] (#2) {$\times$};
}
\newcommand{\wprodnode}[3][]{
  \node[prod, #1] (#2) {$\color{#3}\times$};
}

% \maxnode [tikz-options] {max node name} 
\newcommand{\maxnode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {\scriptsize $max$};
}

% \emptynode [tikz-options] {generic node name}
\newcommand{\emptynode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {};
}

\newcommand{\varnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\varsqnode}[4][]{
  \node[rectangle, rounded corners=3pt,fill=white,draw=#4,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\evnode}[4][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt, #1] (#2) {#3};
}

\newcommand{\evnodevar}[5][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt,
  #1] (#2) {#3};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#5};
}

\newcommand{\bernode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\bernodeleft}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[left=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\bernodedown}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, yshift=1pt] (#2_vn) {#3};
}

\DeclareDocumentCommand{\contnode}{o m m o}  
{%
  \IfNoValueTF{#4}
  {\contnodebelow[#1]{#2}{#3}}
  {\contnodeleft[#1]{#2}{#3}}
}

\newcommand{\contnodebelow}[3][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture}
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\contnodeleft}[3][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} 
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[left=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\catnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] coordinates { (0,0) (0,10)};
                \addplot [mark=none] coordinates { (-1,0) (-1,7)};
                \addplot [mark=none] coordinates { (-2,0) (-2,3)};
                \addplot [mark=none] coordinates { (1,0) (1,5)};
                \addplot [mark=none] coordinates { (2,0) (2,8)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2] (#2_vn) {#3};
}


% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;%
    } ;
  } ;
}

\newcommand{\upedge}[3][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1] (#3);
}

\newcommand{\ledge}[4][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1,edge label=#4] (#3);
}

\newcommand{\weigedge}[4][]{
  \draw[line width=0.6pt,-,#1] (#2) edge node [midway,line width=0.6pt,#1] {#4} (#3) ;
}

\newcommand{\colorweigedge}[7][]{
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;
      % \draw[rounded corners] ($(\x)!0.5!(\y)$) rectangle node{#4} (\y) ;
      \pgfmathparse{width("\noexpand\noexpand\noexpand#4")} ; %the width calc
      \pgfmathsetlength{\mywidth}{\pgfmathresult} ; % Put it into a length register
      \pgfmathparse{height("\noexpand\noexpand\noexpand#4")} ; %the height calc
      \pgfmathsetlength{\myheight}{\pgfmathresult} ; % Put it into a length register
      \node[rectangle,draw,rounded corners=0.4\myheight,line width=0.6pt,color=#5,fill=#6,text=#7,minimum height=1.8\myheight,minimum width=1.2\mywidth,label={center:\textcolor{#7}{#4}}] at ($(\x)!0.5!(\y)$) {} ;
    } ;
  } ;
}

\newcommand{\ellipsis}[2]{
  \node at ($(#1)!.5!(#2)$) {\ldots} ;
}

\newcommand{\annotatenode}[4]{
  \node[] at ([xshift=#3,yshift=#4]#1) {#2} ;
}

\newcommand{\colorfulannotnode}[6]{
  \pgfmathparse{width("\noexpand\noexpand\noexpand#2")} ; %the width calc
  \pgfmathsetlength{\mywidth}{\pgfmathresult} ; % Put it into a length register
  \pgfmathparse{height("\noexpand\noexpand\noexpand#4")} ; %the height calc
  \pgfmathsetlength{\myheight}{\pgfmathresult} ;
  \node[rectangle,draw,rounded corners=0.4\myheight,line width=0.6pt,color=#5,fill=#5,text=#6,minimum height=1.3\myheight,minimum width=1.3\mywidth,label={center:\textcolor{#6}{#2}}] at ([xshift=#3,yshift=#4]#1) {} ;
}

\newcommand{\midlinewidth}{1.0pt}
\newcommand{\incmidlinewidth}{1.7pt}
\newcommand{\largelinewidth}{1.9pt}
\newcommand{\xlargelinewidth}{2.3pt}
\newcommand{\middist}{17pt}
\newcommand{\sqintermiddist}{15.5pt}
\newcommand{\intermiddist}{30pt}
\newcommand{\largedist}{49pt}
\newcommand{\midsmalldist}{10pt}
\newcommand{\smalldist}{6pt}
\newcommand{\tinydist}{4pt}
\newcommand{\centraldist}{30pt}
\newcommand{\midlargedist}{24pt}
\newcommand{\halfdist}{19pt}
\newcommand{\weightsize}{\fontsize{10}{10}\selectfont}
\newcommand{\annotsize}{\fontsize{10}{10}\selectfont}

\definecolor{lacamlilac} {RGB} {107,93,153}
\definecolor{lacamlilac2} {RGB} {93, 109, 152}
\definecolor{lacamlightlilac} {RGB} {174, 166, 201}
\definecolor{lacamdarklilac} {RGB} {51, 10, 102}
\definecolor{lacamdarklilac5} {RGB} {51, 10, 102}
\colorlet{lacamdarklilac4} {lacamdarklilac5!80!}
\colorlet{lacamdarklilac3} {lacamdarklilac5!60!}
\colorlet{lacamdarklilac2} {lacamdarklilac5!40!}
\colorlet{lacamdarklilac1} {lacamdarklilac5!20!}

\definecolor{lacamgold5} {RGB} {255, 87, 0}
\colorlet{lacamgold4} {lacamgold5!80!}
\colorlet{lacamgold3} {lacamgold5!60!}
\colorlet{lacamgold2} {lacamgold5!40!}
\colorlet{lacamgold1} {lacamgold5!20!}
\definecolor{violet} {RGB} {119, 111, 178}
\definecolor{petroil2} {RGB} {36, 165, 175}
\definecolor{petroil4} {RGB} {30, 132, 149}
\definecolor{petroil6} {RGB} {23, 101, 115}
\definecolor{gold2} {RGB} {255, 130, 0}
\definecolor{gold4} {RGB} {250, 100, 0}
\definecolor{gold6} {RGB} {245, 90, 0}

\definecolor{lacamoil5}{rgb}{0.13, 0.67, 0.8}
\colorlet{lacamoil4} {lacamoil5!80!}
\colorlet{lacamoil3} {lacamoil5!60!}
\colorlet{lacamoil2} {lacamoil5!40!}
\colorlet{lacamoil1} {lacamoil5!20!}



%\definecolor{tomato0} {HTML} {E57373}
\definecolor{tomato0} {HTML} {EF9A9A}
\definecolor{tomato1} {HTML} {F44336}
\definecolor{tomato2} {HTML} {E53935}
\definecolor{tomato3} {HTML} {D32F2F}
\definecolor{tomato4} {HTML} {C62828}
\definecolor{tomato5} {HTML} {B71C1C}


\definecolor{peas1} {HTML} {009688}
\definecolor{peas2} {HTML} {00897B}
\definecolor{peas3} {HTML} {00796B}
\definecolor{peas4} {HTML} {00695C}
\definecolor{peas5} {HTML} {004D40}

\definecolor{bgrey0} {HTML} {78909C}
\definecolor{bgrey1} {HTML} {607D8B}
\definecolor{bgrey2} {HTML} {546E7A}
\definecolor{bgrey3} {HTML} {455A64}
\definecolor{bgrey4} {HTML} {37474F}
\definecolor{bgrey5} {HTML} {263238}

\definecolor{olive0} {HTML} {C5E1A5}
\definecolor{olive1} {HTML} {AED581}
\definecolor{olive2} {HTML} {9CCC65}
\definecolor{olive3} {HTML} {8BC34A}
\definecolor{olive4} {HTML} {7CB342}
\definecolor{olive5} {HTML} {689F38}

\definecolor{pink0} {HTML} {FCE4EC}
\definecolor{pink1} {HTML} {F8BBD0}
\definecolor{pink2} {HTML} {F48FB1}
\definecolor{pink3} {HTML} {F06292}
\definecolor{pink4} {HTML} {EC407A}
\definecolor{pink5} {HTML} {FF80AB}

\definecolor{brown0} {HTML} {D7CCC8}
\definecolor{brown1} {HTML} {BCAAA4}
\definecolor{brown2} {HTML} {A1887F}
\definecolor{brown3} {HTML} {8D6E63}
\definecolor{brown4} {HTML} {795548}
\definecolor{brown5} {HTML} {6D4C41}
\definecolor{brown6} {HTML} {5D4037}

\definecolor{yellow0} {HTML} {CDDC39}
\definecolor{yellow1} {HTML} {9E9D24}
\definecolor{yellow3} {HTML} {FFBD2A}
\definecolor{yellow4} {HTML} {FFB000}
\definecolor{yellow5} {HTML} {FFD600}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

==> tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\ProvidesFile{tikzlibrarytikzmark.code.tex}[%
  2021/02/16
  v1.10
  TikZ library for marking positions in a document]
\RequirePackage{expl3, l3keys2e, xparse}
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
          \string\savepicturepage%
          {\pgfpictureid}{\noexpand\arabic{page}}%
        }%
      }%
      \pgf@temp
      \fi%
    },
  },
  check picture id/.code={
    \ifpgfrememberpicturepositiononpage
    \@ifundefined{pgf@sys@pdf@mark@pos@\pgfpictureid}{%
      \tikzset{%
        name prefix/.get=\tzmk@name@prefix,
        name prefix/.prefix=discard-,
        execute at end picture={%
          \tikzset{name prefix/.expand once=\tzmk@name@prefix}%
        },
      }%
    }{}%
    \fi
  },
  maybe define node/.style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage
      \@ifundefined{pgf@sh@pi@\tikz@pp@name{#1}}{%
        \pgfnodealias{\tikz@pp@name{#1}}{discard-\tikz@pp@name{#1}}%
      }{}%
      \fi
    }%
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
      \string\savepointas%
      {\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  if tikzmark on current page/.code n args={3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{%
      \@ifundefined{%
        save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname
      }{%
        \pgfkeysalso{#3}%
      }{%
        \ifnum\csname save@pg@%
        \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
        \endcsname=\the\value{page}\relax%
        \pgfkeysalso{#2}%
        \else
        \pgfkeysalso{#3}%
        \fi
      }%
    }%
  },
  if tikzmark on page/.code n args={4}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#4}%
    }{%
      \@ifundefined{%
        save@pg@\csname save@pt@\tikzmark@pp@name{#1}@label\endcsname%
      }{%
        \pgfkeysalso{#4}%
      }{%
        \ifnum\csname save@pg@%
        \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
        \endcsname=#2\relax%
        \pgfkeysalso{#3}%
        \else
        \pgfkeysalso{#4}%
        \fi
      }%
    }%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{%
  \csname pgfk@/tikz/tikzmark prefix\endcsname%
  #1%
  \csname pgfk@/tikz/tikzmark suffix\endcsname%
}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname%
  {\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\@tikzmarkalias#1#2{%
  \@ifundefined{save@pt@#2}{}{%
    \pgf@node@gnamelet{save@pt@#1}{save@pt@#2}%
    \pgf@node@gnamelet{save@pt@#1@offset}{save@pt@#2@offset}%
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas%
      {#1}{\csname save@pt@#2\endcsname}\expandafter\expandafter\expandafter\@gobble\csname save@pt@#2@offset\endcsname}%
  }%
}
\def\tikzmarkalias#1#2{%
  \@tikzmarkalias{\tikzmark@pp@name{#1}}{\tikzmark@pp@name{#2}}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
    \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}%
    \save@orig@pic%
    \pgfsys@getposition{\pgfpictureid}\save@this@pic%
    \pgf@process{\pgfpointorigin\save@this@pic}%
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\save@orig@pic}%
    \advance\pgf@x by -\pgf@xa
    \advance\pgf@y by -\pgf@ya
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process%
    {\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
        \edef\tmk@pg{%
          \the\numexpr \csname save@pg@%
          \csname save@pt@\tmk@label\endcsname\endcsname%
          -
          \csname save@pg@\pgfpictureid\endcsname\relax%
        }%
        \ifnum \tmk@pg > 0 \relax
        \advance \pgf@xa by \pgf@x\relax
        \advance \pgf@ya by \pgf@y\relax
        \fi
        \ifnum \tmk@pg < 0 \relax
        \advance \pgf@xa by -\pgf@x\relax
        \advance \pgf@ya by -\pgf@y\relax
        \fi
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
  }%
}
\newcommand\tikzmark@outside[2][]{%
\tikzset{external/export next/.try=false}%
\tikz[remember picture with id=#2]{#1}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas%
    {\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x}{\the\pgf@y}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \relax
  \ifx\scope\tikz@origscope\relax
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\arabic{page}}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark@outside}[2][]{%
    \only#3{\beameroriginal{\tikzmark@outside}[{#1}]{#2}}%
  }
  \renewcommand<>{\tikzmark@inside}[2]{%
    \only#3{\beameroriginal{\tikzmark@inside}{#1}{#2}}%
  }
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newif\iftikzmark@
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      #3%
    }{%
      #2%
    }%
}%
\newcommand\iftikzmarkexists[1]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false%
  }{%
    \tikzmark@true%
  }%
  \iftikzmark@
}%
\newcommand\iftikzmarkonpage[2]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false
  }{%
    \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
      \tikzmark@false
    }{%
      \ifnum\csname save@pg@%
      \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
      \endcsname=#2\relax%
      \tikzmark@true
      \else
      \tikzmark@false
      \fi
    }%
  }%
  \iftikzmark@
}
\newcommand\iftikzmarkoncurrentpage[1]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false
  }{%
    \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
      \tikzmark@false
    }{%
      \ifnum\csname save@pg@%
      \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
      \endcsname=\the\value{page}\relax%
      \tikzmark@true
      \else
      \tikzmark@false
      \fi
    }%
  }%
  \iftikzmark@
}
\def\subnode@#1#2#3{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  {%
    \let\pgf@sh@savedmacros=\pgfutil@empty% MW
    \let\pgf@sh@savedpoints=\pgfutil@empty%
    \def\pgf@sm@shape@name{rectangle}% CJ % TT added prefix!
    \pgf@sh@s@rectangle%
    \pgf@sh@savedpoints%
    \pgf@sh@savedmacros% MW
    \pgftransformshift{%
      \pgf@sh@reanchor{rectangle}{center}%
      \pgf@x=-\pgf@x%
      \pgf@y=-\pgf@y%
    }%
    \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
      \pgf@sh@reanchor{rectangle}{center}% FIXME : this is double work!
    }%
    % Save the saved points and the transformation matrix
    \edef\pgf@node@name{\tikz@fig@name}%
    \ifx\pgf@node@name\pgfutil@empty%
    \else%
    \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{rectangle}%
    \edef\pgf@sh@@temp{%
      \noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
    \expandafter\pgf@sh@@temp\expandafter{%
      \pgf@sh@savedpoints}%
    \edef\pgf@sh@@temp{%
      \noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
    \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
    \pgfgettransform\pgf@temp
    \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
    \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
    \fi%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}

\newcommand\subnode[3][]{%
  \ifmmode
  \mathchoice{%
    \subnode@{#1}{#2-d}{\(\displaystyle #3\)}%
  }{%
    \subnode@{#1}{#2-t}{\(\textstyle #3\)}%
  }{%
    \subnode@{#1}{#2-s}{\(\scriptstyle #3\)}%
  }{%
    \subnode@{#1}{#2-ss}{\(\scriptscriptstyle #3\)}%
  }%
  \let\pgf@nodecallback\pgfutil@gobble
  \def\tzmk@prfx{pgf@sys@pdf@mark@pos@pgfid}%
  \edef\tzmk@pic{\tzmk@prfx\the\pgf@picture@serial@count}
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-1\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-2\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-3\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \pgfutil@ifundefined{pgf@sh@ns@#2}{%
    \pgfnodealias{#2}{#2-t}%
    \@tikzmarkalias{#2}{#2-t}%
  }{}%
  \else
    \pgfnodealias{#2}{#2-d}%
    \@tikzmarkalias{#2}{#2-d}%
  \fi
  \else
    \pgfnodealias{#2}{#2-t}%
    \@tikzmarkalias{#2}{#2-t}%
  \fi
  \else
    \pgfnodealias{#2}{#2-s}%
    \@tikzmarkalias{#2}{#2-s}%
  \fi
  \else
    \pgfnodealias{#2}{#2-ss}%
    \@tikzmarkalias{#2}{#2-ss}%
  \fi
  \else
    \subnode@{#1}{#2}{#3}%
  \fi
}

\def\tikzmarknode@#1#2#3{%
\tikzset{external/export next/.try=false}%
  \tikz[%
    remember picture,
    save picture id={#2},
    check picture id,
    maybe define node={#2},
    baseline=(#2.base),
    every tikzmarknode picture/.try
  ] {
    \node[
      anchor=base,
      inner sep=0pt,
      minimum width=0pt,
      name={#2},
      node contents={#3},
      every tikzmarknode/.try,
      #1
  ]}%
}

\newcommand\tikzmarknode[3][]{%
  \ifmmode
  \mathchoice{%
    \tikzmarknode@{#1}{#2-d}{\(\displaystyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-t}{\(\textstyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-s}{\(\scriptstyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-ss}{\(\scriptscriptstyle #3\)}%
  }%
  \let\pgf@nodecallback\pgfutil@gobble
  \def\tzmk@prfx{pgf@sys@pdf@mark@pos@pgfid}%
  \edef\tzmk@pic{\tzmk@prfx\the\pgf@picture@serial@count}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-1\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-2\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-3\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \pgfutil@ifundefined{pgf@sh@ns@\tikz@pp@name{#2}}{%
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-t}}%
    \@tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-t}}%
  }{}%
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-d}}%
    \@tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-d}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-t}}%
    \@tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-t}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-s}}%
    \@tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-s}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-ss}}%
    \@tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-ss}}%
  \fi
  \else
    \tikzmarknode@{#1}{#2}{#3}%
  \fi
}
\def\usetikzmarklibrary{%
  \pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}%
  }%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let%
      \csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

\ExplSyntaxOn
\prop_new:N \g__sn_prop
\tl_new:N \l__sn_tmpa_tl
\tl_new:N \l__sn_tmpb_tl
\tl_new:N \l__open_bracket_tl
\tl_set:Nn  \l__open_bracket_tl {[} %]
\tl_new:N \l__sn_group_tl
\clist_new:N \l__sn_nodes_clist
\bool_new:N \l__sn_file_bool
\bool_new:N \g__sn_preamble_bool
\bool_set_true:N \g__sn_preamble_bool
\msg_new:nnn {tikzmark} {no file} {File~ "#1"~ doesn't~ exist.}
\msg_new:nnn {tikzmark} {loading nodes} {Loading~ nodes~ from~ "#1".}
\dim_new:N \l__sn_x_dim
\dim_new:N \l__sn_y_dim
\dim_new:N \l__sn_xa_dim
\dim_new:N \l__sn_ya_dim
\tl_new:N \l__sn_centre_tl

\tl_new:N \l__sn_transformation_tl
\tl_set:Nn \l__sn_transformation_tl {{1}{0}{0}{1}{0pt}{0pt}}
\iow_new:N \g__sn_stream
\bool_new:N \g__sn_stream_bool
\tl_new:N \g__sn_filename_tl
\tl_gset:Nx \g__sn_filename_tl {\c_sys_jobname_str}

\cs_new_nopar:Npn \sn_open_stream:
{
  \bool_if:NF \g__sn_stream_bool
  {
    \iow_open:Nn \g__sn_stream {\tl_use:N \g__sn_filename_tl .nodes}
    \bool_gset_true:N \g__sn_stream_bool
  }
}

\AtEndDocument
{
  \ExplSyntaxOn
  \bool_if:NT \g__sn_stream_bool
  {
    \iow_close:N \g__sn_stream
  }
  \ExplSyntaxOff
}
\makeatletter
\cs_set_eq:NN \tikz_set_node_name:n \tikz@pp@name
\cs_set_eq:NN \tikz_fig_must_be_named: \tikz@fig@mustbenamed

\cs_new_nopar:Npn \tikz_scan_point:n #1
{
  \tikz@scan@one@point\pgfutil@firstofone#1\relax
}

\cs_new_nopar:Npn \tikz_scan_point:NNn #1#2#3
{
  \tikz@scan@one@point\pgfutil@firstofone#3\relax
  \dim_set_eq:NN #1 \pgf@x
  \dim_set_eq:NN #2 \pgf@y
}

\makeatother
\cs_generate_variant:Nn \tikz_scan_point:n {V}
\cs_generate_variant:Nn \tikz_scan_point:NNn {NNV}
\cs_new_nopar:Npn \save_nodes:Nn #1#2
{
  \tl_clear:N \l__sn_tmpa_tl
  \tikz_scan_point:NNn \l__sn_x_dim \l__sn_y_dim {(current~ bounding~ box.center)}
  \dim_set:Nn \l__sn_x_dim {-\l__sn_x_dim}
  \dim_set:Nn \l__sn_y_dim {-\l__sn_y_dim}
  \tl_set:Nx \l__sn_centre_tl {
    {1}{0}{0}{1}{\dim_use:N \l__sn_x_dim}{\dim_use:N \l__sn_y_dim}
  }
  \clist_map_inline:nn {#2}
  {
    \tl_if_exist:cT {pgf@sh@ns@##1}
    {
      \clist_map_inline:nn {ns,np,ma,pi}
      {
        \tl_put_right:Nn \l__sn_tmpa_tl
        {
          \tl_gset:cn {pgf@sh@####1@ \tikz_set_node_name:n{##1} }
        }
        \tl_if_exist:cTF {pgf@sh@####1@##1}
        {
          \tl_put_right:Nx \l__sn_tmpa_tl {
            {\exp_not:v {pgf@sh@####1@ \tikz_set_node_name:n {##1}}}
          }
        }
        {
          \tl_put_right:Nx \l__sn_tmpa_tl {{}}
        }
      }
      \tl_put_right:Nn \l__sn_tmpa_tl
      {
        \tl_gset:cn {pgf@sh@nt@ \tikz_set_node_name:n{##1} }
      }
      \compose_transformations:NVv \l__sn_tmpb_tl \l__sn_centre_tl {pgf@sh@nt@##1}
      \tl_put_right:Nx \l__sn_tmpa_tl {{\exp_not:V \l__sn_tmpb_tl}}
      \tl_put_right:Nn \l__sn_tmpa_tl {
        \transform_node:Nn \l__sn_transformation_tl {
          \tikz_set_node_name:n{##1}
        }
      }
    }
  }
  \tl_set_eq:NN #1 \l__sn_tmpa_tl
}
\cs_new_nopar:Npn \save_nodes_to_list:nn #1#2
{
  \save_nodes:Nn \l__sn_tmpa_tl {#2}
  \prop_gput:NnV \g__sn_prop {#1} \l__sn_tmpa_tl
}
\cs_new_nopar:Npn \save_nodes_to_file:n #1
{
  \save_nodes:Nn \l__sn_tmpa_tl {#1}
  \sn_open_stream:
  \iow_now:Nx \g__sn_stream
  {
    \iow_newline:
    \exp_not:V \l__sn_tmpa_tl
    \iow_newline:
  }
}
\cs_generate_variant:Nn \save_nodes_to_list:nn {VV}
\cs_generate_variant:Nn \save_nodes_to_file:n {V}
\cs_new_nopar:Npn \restore_nodes_from_list:n #1
{
  \prop_get:NnNT \g__sn_prop {#1} \l__sn_tmpa_tl
  {
    \tl_use:N \l__sn_tmpa_tl
  }
}
\cs_new_nopar:Npn \restore_nodes_from_file:n #1
{
  \file_if_exist:nTF {#1.nodes}
  {
    \msg_log:nnn {tikzmark} {loading nodes} {#1}
    \ExplSyntaxOn
    \file_input:n {#1.nodes}
    \ExplSyntaxOff
  }
  {
    \msg_warning:nnn {tikzmark} {no file} {#1}
  }
}
\AtBeginDocument{\bool_gset_false:N \g__sn_preamble_bool}

\cs_new_nopar:Npn \compose_transformations:Nnn #1#2#3
{
  \tl_gset:Nx #1
  {
    {\fp_eval:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {1}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {2}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {1}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {2}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {3}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {4}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {3}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {4}
      }
    }
    {\fp_to_dim:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {5}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {6}
        +
        \tl_item:nn {#2} {5}
      }
    }
    {\fp_to_dim:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {5}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {6}
        +
        \tl_item:nn {#2} {6}
      }
    }
  }
}
\cs_generate_variant:Nn \compose_transformations:Nnn {cVv,NVv,NVn,NvV,NnV}
\cs_new_nopar:Npn \transform_node:Nn #1#2
{
  \compose_transformations:cVv {pgf@sh@nt@#2} #1 {pgf@sh@nt@#2}
}
\cs_new_nopar:Npn \set_transform_from_node:n #1
{
  \tl_set_eq:Nc \l__sn_transformation_tl {pgf@sh@nt@#1}
  \tikz_scan_point:NNn \l__sn_x_dim \l__sn_y_dim {(#1.center)}

  \dim_set:Nn \l__sn_x_dim {\l__sn_x_dim - \tl_item:cn {pgf@sh@nt@#1}{5}}
  \dim_set:Nn \l__sn_y_dim {\l__sn_y_dim - \tl_item:cn {pgf@sh@nt@#1}{6}}

  \compose_transformations:NnV  \l__sn_transformation_tl {
    {1}{0}{0}{1}{\dim_use:N \l__sn_x_dim}{\dim_use:N \l__sn_y_dim}
  } \l__sn_transformation_tl
}
\cs_generate_variant:Nn \set_transform_from_node:n {v}
\tikzset{
  set~ saved~ nodes~ file~ name/.code={
    \tl_gset:Nx \g__sn_filename_tl {#1}
  },
  transform~ saved~ nodes/.code={
    \set_transform_from_node:v {tikz@last@fig@name}
  },
  set~ node~ group/.code={
    \tl_set:Nn \l__sn_group_tl {#1}
    \pgfkeysalso{
      execute~ at~ end~ scope={
        \maybe_save_nodes:
      }
    }
  },
  save~ nodes~ to~ file/.code={
    \tl_if_eq:nnTF {#1}{false}
    {
      \bool_set_false:N \l__sn_file_bool
    }
    {
      \bool_set_true:N \l__sn_file_bool
    }
    \pgfkeysalso{
      execute~ at~ end~ scope={
        \maybe_save_nodes:
      }
    }
  },
  save~ node/.code={
    \tikz_fig_must_be_named:
    \pgfkeysalso{append~ after~ command={
        \pgfextra{
          \clist_gput_right:Nv \l__sn_nodes_clist {tikz@last@fig@name}
        }
      }
    }
  },
  restore~ nodes~ from~ file/.code={
    \bool_if:NTF \g__sn_preamble_bool
    {
      \restore_nodes_from_file:n {#1}
    }
    {
      \tikz_fig_must_be_named:
      \pgfkeysalso{append~ after~ command={
          \pgfextra{
            \scope
            \split_argument:NNn \tikzset \restore_nodes_from_file:n {#1}
            \endscope
          }
        }
      }
    }
  },
  restore~ nodes~ from~ file/.default = \g__sn_filename_tl,
  restore~ nodes~ from~ list/.code={
    \tikz_fig_must_be_named:
    \pgfkeysalso{append~ after~ command={
        \pgfextra{
          \scope
          \split_argument:NNn \tikzset \restore_nodes_from_list:n {#1}
          \endscope
        }
      }
    }
  }
}
\cs_generate_variant:Nn \clist_gput_right:Nn {Nv}
\cs_new_nopar:Npn \split_argument:NNn #1#2#3
{
  \tl_set:Nx \l__sn_tmpa_tl {\tl_head:n {#3}}
  \tl_if_eq:NNTF \l__sn_tmpa_tl \l__open_bracket_tl
  {
    \split_argument_aux:NNp #1#2#3
  }
  {
    #2 {#3}
  }
}
\cs_new_nopar:Npn \split_argument_aux:NNp #1#2[#3]#4
{
  #1 {#3}
  #2 {#4}
}
\cs_new_nopar:Npn \maybe_save_nodes:
{
  \clist_if_empty:NF \l__sn_nodes_clist
  {
    \bool_if:NTF \l__sn_file_bool
    {
      \save_nodes_to_file:V \l__sn_nodes_clist
    }
    {
      \tl_if_empty:NF \l__sn_group_tl
      {
        \save_nodes_to_list:VV \l__sn_group_tl \l__sn_nodes_clist
      }
    }
    \clist_gclear:N \l__sn_nodes_clist
  }
}
\ExplSyntaxOff
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.


==> tikzmarklibrarylistings.code.tex <==
%%
%% This is file `tikzmarklibrarylistings.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `listings')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\@ifpackageloaded{listings}{%
  \newif\iflst@linemark
  \lst@linemarktrue
\lst@AddToHook{EveryLine}{%
  \begingroup
  \advance\c@lstnumber by 1\relax
  \pgfmark{line-\lst@name-\the\c@lstnumber-start}%
  \endgroup
}
\lst@AddToHook{EOL}{\pgfmark{line-\lst@name-\the\c@lstnumber-end}%
\global\lst@linemarktrue
}
\lst@AddToHook{OutputBox}{%
  \iflst@linemark
  \pgfmark{line-\lst@name-\the\c@lstnumber-first}%
  \global\lst@linemarkfalse
  \fi
}
\def\tkzmk@lst@fnum#1\relax#2\@STOP{%
  \def\@test{#2}%
  \ifx\@test\@empty
  \def\tkzmk@lst@start{0}%
  \else
  \@tempcnta=#1\relax
  \advance\@tempcnta by -1\relax
  \def\tkzmk@lst@start{\the\@tempcnta}%
  \fi
}
\lst@AddToHook{Init}{%
  \expandafter\tkzmk@lst@fnum\lst@firstnumber\relax\@STOP
  \pgfmark{line-\lst@name-\tkzmk@lst@start-start}%
}
}{%
    \PackageError{tikzmark listings}{The listings package has not been loaded.}{}
}
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzmarklibrarylistings.code.tex'.

